Comfort-Aware Building Climate Control Using Distributed-Parameter Models

Controlling Heating, Ventilation and Air Conditioning (HVAC) system to maintain occupant's indoor thermal comfort is important to energy-efficient buildings and the development of smart cities. In this paper, we formulate a model predictive controller (MPC) to make optimal control strategies to HVAC in order to maintain occupant's comfort by predicted mean vote index, and then present a whole system with an estimator to indoor climate and apartment's geometric information based on only thermostats. In order to have accurate spatial resolution and make the HVAC system focus on only a zoned area around the occupant, a convection-diffusion Computer Fluid Dynamics (CFD) model is used to describe the indoor air flow and temperature distribution. The MPC system generates corresponding PDE-constrained optimization problems, and we solve them by obtain the gradients of cost functions with respect to problems' variables with the help of CFD model's adjoint equations. We evaluate the performance of our method using simulations of a real apartment in the St.\ Louis area. Our results show our MPC system's energy efficiency and the potential for its application in real-time operation of high-performance buildings.

==> sections/bios.tex <==
\begin{IEEEbiography}
[{\includegraphics[width=1in,clip,keepaspectratio]{figures/runxin.jpg}}]%
  {Runxin He}
  (S'16) received the B.S.\ degree in electrical
  engineering from Fudan University, Shanghai, China, in 2012, and
  the M.S.\ and Ph.D.\ degrees in electrical engineering
  from Washington University in Saint Louis, MO, USA, in 2017.

  His research focuses on the development and application of novel
  numerical methods to operation research and data science applications. 
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/humberto.jpg}}]%
  {Humberto Gonzalez}
  (S'03-M'12) received the B.S.\ and M.S.\ degrees in electrical engineering from Universidad de Chile, Santiago, Chile, in 2005, and the Ph.D.\ degree in electrical engineering and computer sciences from the University of California at Berkeley, CA, USA, in 2012.
  He is currently a Senior Data Scientist at Instart Logic.

  His research focuses on the development and application of novel
  numerical methods to data science applications. 
\end{IEEEbiography}

% insert where needed to balance the two columns on the last page with
% biographies
%\newpage

% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}


==> sections/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

In this paper, we develop a MPC system to control the thermal comfort around indoor residents based on distributed CFD model.
In order to fulfill this task, we develop a projected gradient-based optimization method to solve related PDE-constrained optimization problems.
The simulation section validate the performance of our MPC to estimate state changes and adapt its control strategy.
Also we studied the influence of personal variables to thermal comfort and MPC system's energy usage, which points out that in order to make the HVAC system energy efficient to thermal comfort control, it is necessary to use some devices to measure occupant's personal variable data.
In the future, based on the memory and time usage studies, in order to speed up our MPC and make it work in real-time, model reduction method will be studied for related PDE-constraint optimization problems.


==> sections/fem_convergence.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Finite Element Approximation}
\label{appendix:fem_appro}
% assumption
% approximation theorem
% where is it comes from
The finite element discretization of a partial derivative is defined as follows.
Define a discritized and finite dimensional subspace for a space,
$S\p{\Omega}$, as $S^h \p{\Omega}$.
%% $T^h \subset H^1(\Omega)$,
%% $V^h \subset H^1(\Omega) \times H^1(\Omega)$
%% and $Q^h \subset L^2(\Omega)$.
Define $L^2_0(\Omega) = \{q \in L^2(\Omega); \, \int_{\Omega} q = 0 \}$.
%% $S_0^h = S^h \cap L^2_0(\Omega)$.
These subspaces are parameterized by a parameter, $h$, which
represents the average size of all discritized elements.
The subspaces usually can be chosen arbitrarily,
while there are some standard discretization assumptions, especially for Navier-Stokes equations.

First, the discrete subspaces should satisfy the assumptions,
there exist an integer $k$ and a constant $C$,
which are independent of each element in the space,
such that, for integer $m \in \sqparen{1, k}$,
\begin{equation}
  \label{eq:app_pro1}
    \inf_{t^h \in H^{m+1, h}\p{\Omega}} \| t - t^h \|_1
    \leq
    C h^m \| t \|_{m+1},
    \,\,
    \forall t \in H^{m+1} (\Omega),
\end{equation}
\begin{equation}
  \label{eq:app_pro2}
  \begin{split}
    & \inf_{v^h \in H^{m+1,h}(\Omega) \times H^{m+1,h}(\Omega)} \| v - v^h \|_1
    \leq
    C h^m \| v \|_{m+1},
    \\
    & \forall v \in H^{m+1}(\Omega) \times H^{m+1}(\Omega),
  \end{split}
\end{equation}
\begin{equation}
  \label{eq:app_pro3}
  \begin{split}
    & \inf_{q^h \in H^{m,h}(\Omega) \cap L^{2,h}_0(\Omega)} \| q - q^h \|_0
    \leq
    C h^m \| q \|_{m},
    \\
    & \forall q \in H^{m}(\Omega) \cap L^2_0(\Omega),
  \end{split}
\end{equation}

Next, we assume the Ladyzhenskaya-Babuska-Brezzi (LBB) condition
holds,
such that there exists a constant $C$, independent of $h$, such that
for non-zero $q^h \in H^{m,h} (\Omega) \cap L^{2,h}_0(\Omega)$,
and non-zero $v^h  \in H^{m+1,h} (\Omega) \times H^{m+1,h}(\Omega)$
\begin{equation}
  \label{eq:lbb_con}
  \inf_{ q^h }
  \sup_{ v^h }
  \frac{b(v^h,q^h)}{\| v^h \|_1 \| q^h \|_0}
  \geq
  C
\end{equation}

Once we have those assumptions, we can discretize the system.
For the heat transfer equation, we discretize the temperature in space first,
then it becomes a series of ODEs.
Here we only estimate the finite element approximation error,
and the time discretized error is not studied.
The discritized system satisfies the discritized weak formulas,
\begin{equation}
  \begin{split}
    & \langle \frac{\partial T_e^h\p{x, t}}{\partial t}, \xi^h\p{x} \rangle_{\Omega}
    - \langle \grad[x]{} \cdot \parenB{ \kappa \grad T_e^h \p{x,t} }, \xi^h\p{x}
    \rangle_{\Omega} + \\
    & + \langle u^h\p{x} \cdot \grad[x]{T_e}^h\p{x,t}, \xi^h\p{x} \rangle_{\Omega}
    - \langle g_{T_e}\p{x,t}, \xi^h\p{x} \rangle_{\Omega}
    = \\
    & = 0, \ \ \forall \xi^h\p{x} \in H^{1, h}\p{\Omega},
  \end{split}
  \label{eq:fem_te}
\end{equation}
\begin{equation}
  \begin{split}
  & \langle \alpha u^h\p{x}, \phi^h\p{x} \rangle_{\Omega}
    + \frac{1}{Re} \langle \grad[x]{u^h}\p{x},\grad[x]{\phi^h\p{x}}
    \rangle_{\Omega} + \\
  & + \langle u^h\p{x} \cdot \grad[x]{u^h\p{x}}, \phi^h\p{x}
    \rangle_{\Omega}
    - \langle p^h\p{x}, \grad[x]{} \cdot \phi^h\p{x} \rangle_{\Omega} +\\
  & - \langle g_u\p{x}, \phi^h\p{x} \rangle_{\Omega}
  = 0, \,\, \forall \phi^h \p{x} \in H^{1, h}\p{\Omega} \times H^{1, h}\p{\Omega},
  \end{split}
  \label{eq:fem_u}
\end{equation}
\begin{equation}
  \langle \grad[x]{\cdot u^h\p{x}}, \psi^h\p{x} \rangle_{\Omega}
  = 0,
  \, \forall \psi^h\p{x} \in L^{2,h}\p{\Omega}
  \label{eq:fum_p}
\end{equation}
with boundary and initial conditions in
equations~\eqref{eq:bnd_t},~\eqref{eq:bnd_u1} and~\eqref{eq:init_t}.

\begin{theorem}
  Suppose $\p{T_e\p{x,t}, u\p{x}, p\p{x}}$ is the solution to the weak form of CFD
  system with
  equations~\eqref{eq:temp} to~\eqref{eq:bnd_u1} in
  Subsection~\ref{subsec:cfd_model}, during the time period
  $t \in \sqparen{t_0, t_0'}$.
  Assume that the finite element spaces $H^{1, h}\p{\Omega}$,
  $H^{1, h}\p{\Omega} \times H^{1, h}\p{\Omega}$ and $L^{2,h} \p{\Omega}$
  satisfy the conditions~\eqref{eq:app_pro1} to~\eqref{eq:lbb_con}.
  Then, for $h$ small enough,
  there exists a tuple $\p{T_e^h\p{x,t}, u^h\p{x}, p^h\p{x}}$ such that
  $T_e^h \p{x,t} \in L^2\p{[t_0, t_0'], H^{1, h} \p{\Omega}}$,
  $u^h \p{x} \in H^{1, h}\p{\Omega} \times H^{1, h}\p{\Omega}$,
  $p^h \p{x} \in L^{2,h} \p{\Omega}$ and $\p{T_e^h\p{x,t}, u^h\p{x}, p^h\p{x}}$
  are the solutions to the discrete system~\eqref{eq:fem_te}
  to~\eqref{eq:fem_u} with corresponding initial and boundary
  conditions.

  Moreover, as $h \rightarrow 0$,
  \begin{align}
    \begin{split}
      & \int_{t_0}^{t_0'} \| T_e\p{\cdot, t} - T_e^h\p{\cdot, t}\|_1 dt \rightarrow 0, \\
      & \| u\p{x} - u^h \p{x} \|_1 \rightarrow 0, \text{ and}\\
      & \| p\p{x} - p^h \p{x} \|_0 \rightarrow 0.
    \end{split}
  \end{align}

  If, in addition, the solution tuple $\p{T_e\p{x,t}, u\p{x}, p\p{x}}$ satisfies,
  \begin{align*}
    \begin{split}
      u\p{x} \in {H}^{m+1}(\Omega) \times {H}^{m+1}(\Omega) \\
      p\p{x} \in L^2(\Omega) \cap H^m(\Omega)
    \end{split}
  \end{align*}
  then there exists constants $C_{1,2,3}$,
  which are independent of $h$, such that
  \begin{align}
    \begin{split}
      & \int_{t_0}^{t_0'} \| T_e\p{\cdot, t} - T_e^h\p{\cdot, t} \|_1 dt
      \leq C_{1} \max \p{ {h}^m, h^2 }, \\
      & \| {u}\p{x} - {u}^h\p{x} \|_1 \leq C_2 h^m, \text{ and} \\
      & \| {p}\p{x} - {p}^h\p{x} \|_0 \leq C_3 h^m.
    \end{split}
  \end{align}
  \label{thm:fem_appr}
\end{theorem}
\begin{IEEEproof}
  Since the temperature and Navier-stokes are weakly coupled,
  the discretization algorithm works as,
  first, we solved the approximated Navier-stokes equation, $u^h$ and $p^h$.
  Then, substitute the $u^h$ into heat transfer equation
  and get the discrete temperature, $T_e^h$.
  As the strategy above, we first estimate the discrete Navier-Stokes.
  The error estimation results can be derived directly
  from~\cite{gunzburger1991analysis} and~\cite{brezzi1980finite},
  concerning the approximation of a class of stationary nonlinear
  problems.

  Then we are going to bound the approximation for $T_e$.
  Substitute $u^h$ into the weak formula for
  equation~\eqref{eq:temp},
  we get
  \begin{equation}
    \begin{split}
      & \langle \frac{\partial T_e \p{x, t}}{\partial t}, \xi\p{x} \rangle_{\Omega}
      - \langle \grad[x]{} \cdot \parenB{ \kappa \grad[x] T_e \p{x, t} }, \xi\p{x}
      \rangle_{\Omega} + \\
      & + \langle u^{{h}}\p{x} \cdot \grad[x]{T_e}\p{x,t}, \xi\p{x} \rangle_{\Omega}
      - \langle g_{T_e}\p{x,t}, \xi\p{x} \rangle_{\Omega} = \\
      & = 0,
      \ \ \  \forall \xi \in H^{1}\p{\Omega}.
  \end{split}
  \label{eq:weak_th}
  \end{equation}
  with initial and boundary condition~\eqref{eq:init_t} and~\eqref{eq:bnd_t}.
  According to theorem~\ref{thm:wk_existence}, there exists a solution
  to the equation~\eqref{eq:weak_th}, define as $T_e^{\tilde h}$.
  Then $\forall t \in (0,T)$,
  \begin{align*}
    & \| T_e(\cdot, t) - T_e^h(\cdot, t) \|_1
    \leq \\
    & \| T_e(\cdot, t) - T_e^{\tilde{h}}(\cdot, t) \|_1
    + \| T_e^{\tilde{h}}(\cdot, t) - T_e^h(\cdot, t) \|_1
  \end{align*}
  Define $e_{t,\tilde{h}}(x, t) = T_e(x, t) - T_e^{\tilde{h}}(x, t)$,
  Substract the weak formula to the equation~\eqref{eq:temp} with the
  equation~\eqref{eq:weak_th},
  $\forall \xi \in H^1(\Omega)$,
  \begin{align}
    \begin{split}
    & \langle \frac{ \partial e_{ t, \tilde{h} } (x, t)}{\partial t}, \xi\p{x} \rangle_{\Omega}
    - \langle \grad[x]{} \cdot \parenB{ \kappa \grad{e_{t,\tilde{h}}(x, t)} },
    \xi \p{x} \rangle_{\Omega} + \\
    & + u\p{x} \cdot \grad[x]{e_{t,\tilde{h}}(x, t)}
    = \\
    & - \langle \paren{ u\p{x} - u^{\tilde{h}}\p{x}} \cdot \grad[x]{Te(x,
      t)}^{\tilde{h}}, \xi\p{x} \rangle_{\Omega},
    \end{split}
    \label{eq:del_te}
  \end{align}
  with zero boundary and initial condition.

  According to linear PDE's energy estimation in~\cite[Theorem 11.1.1]{quarteroni2008numerical},
  \begin{align}
    \| e_{t,\tilde{h}}(\cdot, t) \|_1
    \rightarrow
    0.
    \label{eq:dt_conv}
  \end{align}
  And if the system satisfies the additional assumptions in theorem~\ref{thm:fem_appr},
  there exist constants $C$, which is independent of $h$, such that,
  \begin{align}
    \| e_{t,\tilde{h}}(\cdot, t) \|_1
    \leq
    C {h}^m(t) \paren{
      \|u\|_{m+1}
    },
    \label{eq:dt_conv2}
  \end{align}

  For $\forall t \in \sqparen{t_0, t_0'}$,
  in order to study the error
  $\| T_e^{\tilde{h}} (\cdot, t) - T_e^h(\cdot, t) \|_1$,
  define $e_{t,h}(x, t) = T_e^{\tilde{h}}(x, t) - T_e^h(x, t)$.
  Substract equation~\eqref{eq:weak_th} with~\eqref{eq:fem_te},
  \begin{align}
    \begin{split}
    & \langle \frac{ \partial e_{t,h}(x, t) }{\partial t}, \xi^h\p{x} \rangle_{\Omega}
    - \langle \grad[x]{} \cdot \parenB{ \kappa \grad{e_{t,h}(x, t)} }, \xi^h\p{x}
    \rangle_{\Omega} + \\
    & + \langle u^{\tilde{h}}\p{x} \cdot \grad[x]{ e_{t,h}(x, t) }, \xi^h\p{x} \rangle_{\Omega}
    = 0,
    \, \forall \xi^h\p{x} \in H^{1,h} \p{\Omega},
    \end{split}
    \label{eq:fem_et}
  \end{align}
  With zero boundary and initial conditions.

  For $e_{t,h}\p{x, t}$, choose $\xi^h \p{x} = T_e^h\p{x, t} - w^h\p{x}$,
  $w^h \p{x} \in T^h$,
  then $\xi^h \p{x} = \p{T_e^{\tilde h}\p{x,t} - w^h\p{x}} - e_{t,h}\p{x,t}$,
  separate the equation~\eqref{eq:fem_et} and
  according to Schwartz inequality,
  \begin{align}
    \begin{split}
      & \langle \frac{ \partial e_{t,h}(x, t) }{\partial t},
      e_{t,h}(x, t) \rangle_{\Omega}
      - \langle \grad[x]{} \cdot \parenB{ \kappa \grad{e_{t,h}(x, t)} },
      e_{t,h}(x, t) \rangle_{\Omega} + \\
      & + \langle u^{\tilde{h}}(x) \cdot \grad[x]{ e_{t,h}(x, t) },
      e_{t,h}(x, t) \rangle_{\Omega}
      = \\
      & \langle \frac{ \partial e_{t,h}(x, t) }{\partial t},
      e_{t,h}(x, t) \rangle_{\Omega}
      - \langle \grad[x]{} \cdot \parenB{ \kappa \grad[x]{e_{t,h}}(x, t) },
      \\
      & e_{t,h}(x, t) \rangle_{\Omega}
      =
      %%%%%%%%%%%%%
      %%%%%%%%%%%%%
      - \langle \frac{ \partial e_{t,h}(x, t) }{\partial t},
      T_e^{\tilde h}(x, t) - w^h\p{x} \rangle_{\Omega} + \\
      & + \langle \grad[x]{} \cdot \parenB{ \kappa \grad[x]{e_{t,h}(x, t)} },
      T_e^{\tilde h}(x,t) - w^h\p{x} \rangle_{\Omega} + \\
      & - \langle u^{\tilde{h}}(x) \cdot \grad[x]{ e_{t,h}(x, t) },
      T_e^{\tilde h}(x, t) - w^h\p{x} \rangle_{\Omega}
      \leq \\
      %%%%%%%%%%%%%
      %% & \leq \| \dot{e_{t,h}(t)} \|_0 \| Te(t) - w^h \|_0
      %% + \lambda_1 \| e_{t,h}(t) \|_1 \| Te(t) - w^h \|_1
      %% + \lambda_2 \| u^{\tilde{h}}\|_{\infty} \| e_{t,h}(t) \|_1 \| Te(t) - w^h \|_1
      %% \leq \\
      %%%%%%%%%%%%%%
      & \leq \| \frac{ \partial e_{t,h}(x, t) }{\partial t} \|_0 \|
      T_e^{\tilde h}(x, t) - w^h \p{x} \|_0 + \\
      & + \lambda_1 \| e_{t,h}(x, t) \|_1 \| T_e^{\tilde h}(x, t) - w^h\p{x} \|_1 + \\
      & + \lambda_2 \| u^{\tilde{h}}(x) \|_{\infty} \| e_{t,h}(x, t) \|_1 \|
      T_e^{\tilde h}(x, t) - w^h\p{x} \|_1
      \leq \\
      & \leq \| \frac{ \partial e_{t,h}(x, t) }{\partial t} \|_0 \|
      T_e^{\tilde h}(x, t) - w^h \p{x}\|_0 + \\
      & + \lambda \| e_{t,h}(x, t) \|_1 \| T_e^{\tilde h}(t) - w^h\p{x} \|_1
      \leq \\
      %%%%%%%%%%%%%%
      & \leq \| \frac{ \partial e_{t,h}(x, t) }{\partial t} \|_0
      \| T_e^{\tilde h}(x, t) - w^h\p{x} \|_0 + \\
      & + \frac{ \lambda^2 }{ 4 \epsilon } \| e_{t,h}(x, t) \|^2_1
      + \epsilon \| T_e^{\tilde h}(x, t) - w^h\p{x} \|^2_1
    \end{split}
    \label{eq:err_te_bnd}
  \end{align}
  where $\lambda$ is independent from ${h}$, and $\forall \epsilon > 0$.

  According to lemma~\ref{lem:sigma1_coercive},
  there exists a constant $k$,
  independent of $h$, s.t,
  \begin{equation*}
    \begin{split}
    & - \langle \grad[x]{} \cdot \parenB{ \kappa \grad[x]{e_{t,h}}(x, t) },
    e_{t,h}\p{x, t} \rangle_{\Omega}
    = \\
    & = \langle \kappa \grad[x]{e_{t,h}}(x, t), \grad[x]{e_{t,h}\p{x, t}} \rangle_{\Omega}
    \geq \\
    & \geq k \| e_{t,h} \p{\cdot, t} \|_1^2
    \end{split}
  \end{equation*}
  According to~\cite[Corollary 11.1.1]{quarteroni2008numerical},
  it follows that $T_e^{\tilde h}, w_t \in L^2([t_0,t_0']; H^2(\Omega))$.
  Hence, choosing for almost any $t \in [t_0,t_0']$
  $w^h = \pi^h(T_e^{\tilde h}(t))$,
  the projection of $T_e^{\tilde h}(x, t)$ into
  $H^{1,h}\p{\Omega}$,
  then,
  \begin{align*}
    \| T_e^{\tilde h}(\cdot, t) - w^h \|_0^2
    \leq
    C_{\pi,1} h^2 \|T_e^{\tilde h}(\cdot, t)\|^2_2 \\
    \| T_e^{\tilde h}(\cdot, t) - w^h \|_1^2
    \leq
    C_{\pi,2} h^2 \| T_e^{\tilde h}(\cdot, t) \|^2_2
  \end{align*}

  The initial estimation is zero, i.e.,
  $\| e_{t,h}(\cdot, 0) \|_0^2 = 0$.
  Choose $\epsilon = k / \p{2 \lambda^2}$,
  integrate~\eqref{eq:err_te_bnd} from $t_0$ to $t_0'$,
  there exists a constant, $\tilde{C}_3$,
  independent of $h$,
  \begin{align*}
    \begin{split}
      & k \int_{t_0}^{t_0'} \| e_{t,h}(\cdot, \tau) \|_1^2
      \leq
      \| e_{t,h}(\cdot, t) \|_0^2
      + k \int_{t_0}^{t_0'} \| e_{t,h}(\cdot, \tau) \|_1^2
      \leq \\
      & \leq \tilde{C}_3 h^2 \int_{t_0}^{t_0'}
      (
        \| \frac{\partial T_e^{\tilde h}}{\partial t} (\cdot, \tau) \|_0^2
        + \| \frac{\partial Te^h}{\partial t} (\cdot, \tau) \|^2_0 )
      + \\
      & + \|  T_e^{\tilde h}(\cdot, \tau) \|_2^2 ) d \tau
      %% & = \tilde{C}_3 h^2 \int_0^t \paren{
      %%   \| \frac{\partial Te}{\partial t} (\tau) \|_0^2
      %%   + \| \frac{\partial Te^h}{\partial t} (\tau) \|^2_0
      %%   + \|  Te(\tau) \|_2^2 }
    \end{split}
  \end{align*}
  By~\cite[Proposition 11.1.1]{quarteroni2008numerical},
  $\| \frac{\partial T_e^h}{\partial t} \p{\cdot, t}\|_0^2$ is bounded,
  thus,
  there exists a constant, $C_3$,
  which is independent of $h$, such that,
  \begin{equation}
    \int_{t_0}^{t_0'} \| e_{t,h}(\cdot, \tau) \|_1^2
    \leq
    C_3 h^2
  \end{equation}

  Thus, if the system satisfies the additional assumptions in the theorem~\ref{thm:fem_appr},
  \begin{align}
    \int_{t_0}^{t_0'} \| T_e\p{\cdot, t} - T_e^h\p{\cdot, t} \|_1 dt
    \leq
    C \max \p{\tilde{h}^m, {h}^2}
    \label{eq:err_te}
  \end{align}

\end{IEEEproof}


==> sections/frechet_existence.tex <==
\section{Proof of Fr\'echet Derivatives}
\label{appendix:frechet_proof}

In this section, we prove that the formulas in eqs.~\eqref{eq:i0_deriv}, \eqref{eq:theta_deriv}, \eqref{eq:gte_deriv}, and~\eqref{eq:gu_deriv} are indeed the Fr\'echet derivatives our generalized cost objective function $J$ defined in Sec.~\ref{sec:adj_eq}.
% We are going to show these derivatives are Gateaux derivatives and then extend to show they are Fr\'echet derivatives.

%% \todo{define $[.]$ notation here}
%%%%%%%%%%% I'm here
First, we define the notation for Gateaux derivative.
Let $X$ and $Y$ be Banach spaces and let $f : X \to Y$ be a function between
them.
Given $x \in X$ and a variance $\delta x \in X$, the Gateaux derivative of
function $f$ at point $f(x)$ w.r.t. $\delta x$ is define as $f[\delta x]$.
% \begin{theorem}
%   \label{thm:je_frechet}
%   Let $\pi_0 \in H^1\p{\Omega}$, $\theta \in \R^{n_d}$, and $\alpha, \kappa \in L^2\p{\Omega} \cap L^{\infty}\p{\Omega}$.
%   The directional derivatives in equations~\eqref{eq:i0_deriv} and~\eqref{eq:theta_deriv} are Fr\'echet derivatives of cost function $J_e$ to corresponding variables.
% \end{theorem}

\begin{lemma}
  \label{lem:kappa_derivative}
  The solution to the CFD model in equations~\eqref{eq:temp} to~\eqref{eq:bnd_u1}, $\p{T_e, u, p}$, has a Gateaux derivative $\pb{w_t\sqparen{\delta \kappa}, w_u\sqparen{\delta \kappa}, w_p\sqparen{\delta \kappa}}$  in every direction $\delta \kappa \in L^{\infty}(\Omega) \cap L^2 \p{\Omega}$ w.r.t. $\kappa \in L^{\infty}(\Omega) \cap L^2 \p{\Omega}$.
  Furthermore, the Gateaux Derivatives, $w_u \sqparen{\delta \kappa} = 0$, $w_p \sqparen{\delta \kappa} = 0$ and $w_t \sqparen{\delta \kappa}$ is the solution to the PDE:
  \begin{equation}
    \label{eq:temp_kappa}
    \begin{split}
      & \pderiv{w_t\sqparen{\delta \kappa}}{t}(x,t)
      - \grad[x] \cdot \pb{\delta \kappa \, \grad[x]{T_e}(x,t; \kappa)} + \\
      &- \grad[x] \cdot \pb{\kappa \, \grad[x]{w_t\sqparen{\delta \kappa}}(x,t)}
      + u(x) \cdot \grad[x]{w_t\sqparen{\kappa}}(x,t)
      = 0,
    \end{split}
  \end{equation}
  With initial condition,
  \begin{equation}
    \label{eq:init_t_kappa}
    w_t\sqparen{\delta \kappa} (x, t_0) = 0,\quad \text{for}\ x \in \Omega.
  \end{equation}
  and boundary condition,
  \begin{equation}
    \label{eq:bnd_t_kappa}
    w_t \sqparen{\delta \kappa} (x) \equiv 0,
    \quad \text{for}\ x \in \bdry{\Omega}.
  \end{equation}
\end{lemma}
\begin{IEEEproof}
  Since $\kappa$ does not relate to Navier-Stokes
  equations~\eqref{eq:ns1},~\eqref{eq:ns2} and~\eqref{eq:bnd_t},
  $w_u \sqparen{\delta \kappa} = 0$ and $w_p \sqparen{\delta \kappa} =
  0$.

  Define the weak solution to temperature with given $\kappa$ as
  $T_e \p{x,t; \kappa}$.
  Define $\tilde{T_e}\p{x, t} = T_e(x,t; \kappa + s \delta \kappa) -
  T_e(x,t; \kappa) - sw_{t}\sqparen{t_0, t_0'}$,
  then for $w_{t} \sqparen{\delta \kappa}$,
  it is sufficient to show for $w_{t}\sqparen{\delta \kappa}$ satisfying the following:
  \begin{equation}
    \label{eq:lim_k_wt}
    \lim_{s \to 0} \parenB{
      \frac{\| \tilde{T_e} \|_{\Omega \times
          \sqparen{t_0, t_0'}}}{ |s| } }
    = 0
  \end{equation}

  Define
  $\hat{T_e} = T_e(\kappa + s \delta \kappa) - T_e(\kappa)$,
  then $\tilde{T_e}$ satisfies the following PDE
  \begin{equation}
    \label{eq:tilde_t_k}
    \begin{split}
      & \pderiv{\tilde{T_e}}{t}(x,t)
      + u(x) \cdot \grad[x]{\tilde{T_e}}(x,t)
      - \grad[x] \cdot \pb{\kappa \, \grad[x]{\tilde{T_e}}(x,t)} = \\
      & = s \grad[x] \cdot \pbb{\delta \kappa \,
        \grad[x] \hat{T_e} (x,t)},
    \end{split}
  \end{equation}
  with homogeneous zero initial and boundary conditions.
  $\hat{T_e}$ satisfies the following PDE
  \begin{equation}
    \label{eq:hat_t_k}
    \begin{split}
      & \pderiv{\hat{T_e}}{t}(x,t)
      + u(x) \cdot \grad[x]{\hat{T_e}}(x,t)
      - \grad[x] \cdot \pb{\kappa \, \grad[x]{\hat{T_e}}(x,t)} = \\
      & = s \grad[x] \cdot \pbb{\delta \kappa \,
        \grad[x] T_e \p{x, t; \kappa + s \delta \kappa}},
    \end{split}
  \end{equation}
  also with homogeneous zero initial and boundary conditions.
  According to the energy estimation
  inequality~\cite[Chapter~11.1]{quarteroni2008numerical},
  we can bound $\hat{T_e}$ and $\tilde{T_e}$,
  \begin{equation}
    \norm{\hat{T_e}}_{\Omega \times \sqparen{t_0,t_0'}}
    \leq s C_1 \norm{T_e \p{x, t; \kappa + s \delta \kappa}}_{\Omega \times
      \sqparen{t_0, t_0'}},
  \end{equation}
  \begin{equation}
    \begin{split}
    \norm{\tilde{T_e}}_{\Omega \times \sqparen{t_0,t_0'}}
    \leq s C_2 \norm{\hat{T_e}}_{\Omega \times \sqparen{t_0, t_0'}}
    \leq \\
    \leq s^2 C_1 C_2 \norm{T_e \p{x, t; \kappa + s \delta \kappa}}_{\Omega \times
      \sqparen{t_0, t_0'}},
    \end{split}
  \end{equation}
  where $C_{1,2} > 0$ are two independent parameters.
  Thus equation~\eqref{eq:lim_k_wt} holds and $w_t\sqparen{\delta
    \kappa}$ is $T_e$ Gateaux derivative w.r.t. $\delta \kappa$.
\end{IEEEproof}

\begin{lemma}
  \label{lem:alpha_derivative}
  The solution to the CFD model in equations~\eqref{eq:temp}
  to~\eqref{eq:bnd_u1},
  $\p{T_e, u, p}$ has a Gateaux derivative
  %% $\pb{w_t\sqparen{\delta \alpha}, w_u\sqparen{\delta \alpha},
  %%   w_p\sqparen{\delta \alpha}}$
  in every direction
  $\delta \alpha \in L^{\infty}(\Omega) \cap L^2 \p{\Omega}$ w.r.t.
  $\alpha \in L^{\infty}(\Omega) \cap L^2 \p{\Omega}$.
  Furthermore, the Gateaux Derivatives of $T_e$ and $u$,
  $w_t \sqparen{\delta \alpha}$ and
  $w_u \sqparen{\delta \alpha}$ are the solution to the PDE:
  \begin{equation}
    \label{eq:temp_alpha}
    \begin{split}
      & \pderiv{w_{t}\sqparen{\delta \alpha}\p{x}}{t}
      - \grad[x] \cdot \paren{\kappa \, \grad[x] w_{t}\sqparen{\delta
          \alpha}\p{x}}  + \\
      & + u(x; \alpha) \cdot \grad[x]{w_{t}\sqparen{\delta
          \alpha}\p{x}} + \\
      & + w_{u}\sqparen{\delta \alpha}\p{x} \cdot \grad[x]{T_e(x; \alpha)} = 0,
    \end{split}
  \end{equation}
  \begin{equation}
    \label{eq:ns1_alpha}
    \begin{split}
      & \alpha w_{u}\sqparen{\delta \alpha} \p{x}
      + \delta \alpha u\p{x; \alpha} + \\
      & - \frac{1}{Re} \lapl[x]{w_{u}\sqparen{\delta \alpha}}
      + u(x; \alpha) \cdot \grad[x]{w_{u}\sqparen{\delta \alpha}}\p{x}
      + \\
      & + w_u \sqparen{\delta \alpha} \cdot \grad[x]{u(x; \alpha)}
      + \grad[x]{w_{p}}\p{x}
      = 0, \quad \text{and},
    \end{split}
  \end{equation}
  \begin{equation}
    \label{eq:ns2_alpha}
    \diver[x]{w_u\sqparen{\delta \alpha}}\p{x} = 0,
  \end{equation}
  with homogeneous zero initial and boundary conditions.
\end{lemma}
\begin{IEEEproof}
  First,
  We prove $w_u\sqparen{\delta \alpha}$ above is the Gateaux derivative.
  Define
  $\tilde{u}\p{x} = u(x; \alpha + s \delta \alpha) - u(x; \alpha) - s w_{u} \sqparen{\delta
    \alpha}\p{x}$,
  then it is sufficient to show that,
  \begin{equation}
    \label{eq:lim_wu_alpha}
    \lim_{s \to 0} \parenB{ \frac{\| \tilde{u}\p{x} \|_{1}}{ |s| } } = 0
  \end{equation}
  %% Define
  %% $\tilde{u} = u(\alpha + s \delta \alpha) - u(\alpha) - s w_{u} \sqparen{\delta \alpha}$
  %% $\tilde{p} = p(\alpha + s \delta \alpha) - p(\alpha) - s w_{p}\sqparen{\delta
  %% \alpha}$
  According to~\cite{gunzburger2000adjoint}, $\tilde{u}$ satisfies
  the PDE
  \begin{equation}
    \label{eq:tilde_u_alpha}
    \begin{split}
      & \alpha \tilde{u}\p{x}
      - \frac{1}{Re} \lapl{ \tilde{u}\p{x} }
      + u(x; \alpha) \cdot \grad{\tilde{u}\p{x}}
      + \tilde{u}\p{x} \cdot \grad{u(x; \alpha)}
      = \\
      & = -s \delta \alpha \pb{u(x; \alpha + s \delta \alpha) - u(x; \alpha)}
      + k_u,
    \end{split}
  \end{equation}
  with zero homogeneous boundary condition,
  and $k_u$ is defined as
  \begin{equation}
    \label{eq:ku_alpha}
    \begin{split}
      & k_u =
      - u(x; \alpha + s \delta \alpha) \cdot \grad[x]{u(x; \alpha+s \delta \alpha)} +\\
      & + u(x; \alpha) \cdot \grad[x]{u(x; \alpha + s \delta \alpha )} + \\
      & + u(x; \alpha + s \delta \alpha) \cdot \grad[x]{u\p{x; \alpha}}
      - u(x; \alpha) \cdot \grad[x]{u(x; \alpha)}.
    \end{split}
  \end{equation}
  Multiply both sides of~\eqref{eq:tilde_u_alpha} with $\tilde{u}$ and
  integrate in $\Omega$,
  by the notations and calculations from~\appendixref{appendix:existence},
  %% Section~\ref{subsec:existence},
  we get
  \begin{equation}
    \label{eq:tilde_u_wk}
    \begin{split}
      & \dprod{ \alpha \tilde{u} }{ \tilde{u} }_{\Omega}
      - \dprod{ \frac{1}{Re} \lapl[x]{ \tilde{u} } }{ \tilde{u} }_{\Omega}
      + \dprod{ u(x; \alpha) \cdot \grad[x]{\tilde{u}} }{ \tilde{u} }_{\Omega} + \\
      & + \dprod{ \tilde{u} \cdot \grad[x]{u(x, \alpha)} }{ \tilde{u} }_{\Omega}
      %% %% c_{\alpha} ( \tilde{u}, \tilde{u} )
      %% %% + a_0 ( \tilde{u}, \tilde{u} )
      %% %% + b_0 ( u( u_0 ), \tilde{u}, \tilde{u} )
      %% %% + b_0 ( \tilde{u}, u( u_0 ), \tilde{u} ) = \\
      = \sigma_0 ( \tilde{u}, \tilde{u} ) = \\
      & = \dprod{-s \delta \alpha \pb{u(\alpha + s \delta \alpha) - u(\alpha)} + k_u}
      {\tilde{u}}_{\Omega}
    \end{split}
  \end{equation}
  According to~\appendixref{appendix:existence},
  %% Section~\ref{subsec:existence},
  $\sigma_0$ is a coercive bilinear operator, thus there exists a positive real number $C_1$ s.t
  \begin{equation}
    \begin{split}
      \label{eq:c0_tildeu_alpha}
      & 0
      \leq \| \tilde{u} \|^2_1
      \leq C_1 \sigma_0 (\tilde{u}, \tilde{u})
      = \\
      & = C_1 \dprod{-s \delta \alpha \pb{u(x; \alpha + s \delta \alpha) - u(x; \alpha)} + k_u}
      {\tilde{u}}_{\Omega}
      \leq \\
      & \leq C_1 |\dprod{-s \delta \alpha \pb{u(x; \alpha + s \delta \alpha) -
          u(x; \alpha)}}{\tilde{u}}_{\Omega}| + \\
      & + C_1 |\dprod{k_u}{\tilde{u}}_{\Omega}|.
    \end{split}
  \end{equation}

  In order to prove the equation~\eqref{eq:lim_wu_alpha},
  it is sufficient to prove that the two terms,
  $|\dprod{-s \delta \alpha \pb{u(x; \alpha + s \delta \alpha) - u(x; \alpha)}}{\tilde{u}}_{\Omega}|$
  and $|\dprod{k_u}{\tilde{u}}_{\Omega}|$
  are bounded by higher order of $s$.
  Define $\hat{u} = u(x; \alpha + \delta \alpha) - u(x; \alpha)$,
  then $|\dprod{k_u}{\tilde{u}}_{\Omega}|$ can be bounded as,
  \begin{equation}
    \begin{split}
      & \dprod{k_u}{\tilde{u}}_{\Omega}
      =
      | - \dprod{ u(x; \alpha + s \delta \alpha) \cdot \grad[x]{u(x; \alpha+s \delta \alpha)}}{ \tilde{u}}_{\Omega}
      + \\
      & + \dprod{ u(x; \alpha) \cdot \grad[x]{u(x; \alpha + s \delta \alpha)}}{
        \tilde{u} } + \\
      & + \dprod{ u(x; \alpha+s \delta \alpha) \cdot \grad[x]{u\p{x; \alpha}}}{ \tilde{u} }_{\Omega} + \\
      & - \dprod{ u(x; \alpha) \cdot \grad[x]{u(x; \alpha)}}{ \tilde{u}
      }_{\Omega} | = \\
      & = |
      - \dprod{ \hat{u} \cdot \grad[x]{u(x; \alpha + s \delta \alpha)}}{ \tilde{u} }_{\Omega}
      + \dprod{ \hat{u} \cdot \grad[x]{u(x; \alpha)}}{ \tilde{u} }_{\Omega} |
      = \\
      & = | \dprod{ \hat{u} \cdot \grad[x]{ \hat{u} }}{ \tilde{u} }_{\Omega} |
      \leq \\
      & \leq C_2 |\hat{u}|_1 \| \hat{u} \|_1 \| \tilde{u} \|_1
      \leq C_3 \norm{\hat{u}}_1^2 \norm{\tilde{u}}_1,
    \end{split}
  \end{equation}
  where $C_{2,3} > 0$ and independent of $s$.
  $\hat{u}$ is the solution to the PDE
  \begin{equation}
    \begin{split}
      & \alpha \hat{u}\p{x}
      + s \delta \alpha u(x; \alpha + s \delta \alpha)
      - \frac{1}{Re} \lapl[x]{\hat{u}}\p{x} + \\
      & + u(x; \alpha) \cdot \grad[x]{\hat{u}}\p{x}
      + \hat{u}\p{x} \cdot \grad[x]{u(x; \alpha)} + \\
      & + \hat{u}\p{x} \cdot \grad[x]{\hat{u}}\p{x}
      + \grad[x]{\hat{p}}\p{x}
      = 0, \quad \, \text{and},
    \end{split}
  \end{equation}
  \begin{equation}
    \grad[x] \cdot \hat{u} = 0.
  \end{equation}
  with zero homogeneous boundary condition.

  In order to bound $\hat{u}$,
  we separate it into two values,
  $\hat{u} = \hat{u}_1 + \hat{u}_2$, s.t.,
  \begin{equation}
    \begin{split}
      & \alpha \hat{u}_1\p{x}
      - \frac{1}{Re} \lapl[x]{\hat{u}_1}\p{x}
      + \grad[x]{\hat{p}}\p{x}
      = - s \delta \alpha u(x; \alpha + \delta \alpha),
    \end{split}
    \label{eq:tilde_u1_1}
  \end{equation}
  \begin{equation}
    \begin{split}
      & \grad[x]{} \cdot \hat{u}_1\p{x} = 0,
    \end{split}
    \label{eq:tilde_u1_2}
  \end{equation}
  \begin{equation}
    \begin{split}
    & \alpha \hat{u}_2\p{x}
    - \frac{1}{Re} \lapl[x]{\hat{u}_2}\p{x}
    + (u(x; \alpha) + \hat{u}_1\p{x}) \cdot \grad[x]{\hat{u}_2}\p{x} + \\
    & + \hat{u}_2\p{x} \cdot \grad[x]{ \paren{ u(x; \alpha) + \hat{u}_1\p{x} } }
    + \hat{u}_2\p{x} \cdot \grad[x]{\hat{u}_2}\p{x}
    = \\
    & =
    - \hat{u}_1\p{x} \cdot \grad[x]{u(x; \alpha)}
    - u(x; \alpha) \cdot \grad[x]{\hat{u}_1\p{x}} + \\
    & - \hat{u}_1\p{x} \cdot \grad[x]{\hat{u}_1\p{x}},
    \quad \, \text{and}
    \end{split}
    \label{eq:tilde_u2_1}
  \end{equation}
  \begin{equation}
    \begin{split}
      & \grad{} \cdot \hat{u}_2 = 0.
    \end{split}
    \label{eq:tilde_u2_2}
  \end{equation}
  Both $\hat{u}_1$ and $\hat{u}_2$ are with zero homogeneous boundary
  conditions.

  Similar to the strategy to bound $\tilde{u}$ in
  equation~\eqref{eq:c0_tildeu_alpha},
  we can bound $\hat{u}_1$ by $s$ and $\norm{u(x; \alpha + s \delta \alpha)}$
  as
  $\norm{\tilde{u}_1}_1 \leq C_4 |s \delta \alpha| \norm{u(x; \alpha + s \delta \alpha)}_1$,
  where $C_4 > 0$ is independent of $s$.
  Then for $\hat{u}_2$, we can bound it by $s$ as well,
  $\norm{\tilde{u}_2}_1 \leq C_5 \norm{- \tilde{u}_1 \cdot \grad{u(x; \alpha)} -
  u(x; \alpha) \cdot \grad[x]{\tilde{u}_1} - \tilde{u}_1 \cdot
  \grad[x]{\tilde{u}_1}}_1 \leq C_6 |s| \norm{u(x; \alpha)}_1$,
  where $C_{5,6} > 0$ are independent to $s$.

  Thus the limitation in equation~\eqref{eq:lim_wu_alpha} holds.
  Then we are going to talk about $w_{t}\sqparen{\delta \alpha}$,
  define $\tilde{T_e} = T_e(x,t; \alpha + s \delta \alpha) - Te(x,t; \alpha) -
  sw_{t}$,
  it is sufficient to show that
  \begin{equation}
    \label{eq:lim_wt_alpha}
    \lim_{s \to 0} \parenB{ \frac{ \norm{\tilde{T_e}}_{L^2(0,T; H^1(\Omega))} }{ |s| } } = 0
  \end{equation}
  $\tilde{T_e}$ follows
  \begin{equation}
    \label{eq:tilde_t_alpha}
    \begin{split}
      & \pderiv{\tilde{T_e}}{t}\p{x,t}
      - \grad[x] \cdot \paren{ \kappa \grad[x]{\tilde{T_e}\p{x,t}} } + \\
      & - u(x; \alpha) \cdot \grad[x] \tilde{T_e}\p{x,t}
      = k_t,
      %% + u(\alpha + s \delta \alpha) \cdot \grad{T_e(\alpha+s \delta \alpha)}
      %% + \\
      %% & - u(\alpha) \cdot \grad{T_e(\alpha)}
      %% - u(\alpha) \cdot \grad{s w_t\sqparen{\delta \alpha}}
      %% + \\
      %% & - s w_u\sqparen{\delta \alpha} \cdot \grad{T_e(\alpha)}
      %% = 0
    \end{split}
  \end{equation}
  with zero boundary and initial conditions,
  where $k_t = - \tilde{u} \cdot \grad[x]{T_e(x,t; \alpha + s \delta \alpha)} - s
  w_u\sqparen{\delta \alpha} \cdot \pb{\grad[x]{T_e(x,t; \alpha + s \delta \alpha) -
      T_e(x,t; \alpha)}}$.
  Then according to~\cite[Theorem~11.1.1]{quarteroni2008numerical},
  we can bound $\norm{\tilde{T_e}}_{\Omega \times [t_0,t_0']}$ by
  $\norm{k_t}_{\Omega}$,
  it is sufficient to show that $\norm{k_t}_{\Omega}$ can be bounded
  by higher order of $|s|$.

  Define $\hat{T_e} = T_e(x,t; \alpha + s \delta \alpha) - T_e(x,t; \alpha)$,
  it follows the PDE
  \begin{equation}
    \begin{split}
    & \pderiv{\hat{T_e}}{t}\p{x,t}
    - \grad[x]{} \paren{ \kappa \grad[x]{ \hat{T_e} }\p{x,t} } + \\
    & + u(x; \alpha+s w_u) \cdot \grad[x]{\hat{T_e}}\p{x,t}
    = - \hat{u} \cdot \grad{ T_e(\alpha) }
    \end{split}
    \label{eq:hat_t_alpha}
  \end{equation}
  with zero homogeneous boundary and initial conditions.
  Since $\norm{\hat{u}}_1$ is bounded by $|s|$,
  so does $\norm{\hat{T_e}}_{\Omega \times \sqparen{t_0,t_0'}}$.
  Thus the limitation in equation~\eqref{eq:lim_wt_alpha} holds as well.
\end{IEEEproof}

\begin{lemma}
  \label{lem:pi0_derivative}
  The solution to the CFD model in equations~\eqref{eq:temp}
  to~\eqref{eq:bnd_u1},
  $\p{T_e, u, p}$ has a Gateaux derivative
  %% $\pb{w_t\sqparen{\delta \alpha}, w_u\sqparen{\delta \alpha},
  %%   w_p\sqparen{\delta \alpha}}$
  in every direction
  $\delta \pi_0 \in H^1\p{\Omega}$ w.r.t.
  $\pi_0 \in H^1\p{\Omega}$.
  Furthermore, the Gateaux Derivatives of $T_e$,
  $w_t \sqparen{\delta \pi_0}$ is the solution to the PDE:
  %% $w_u \sqparen{\delta \pi_0}$ and $w_p \sqparen{\delta \pi_0}$
  \begin{equation}
    \label{eq:temp_pi0}
    \begin{split}
      & \pderiv{w_{t}\sqparen{\delta \pi_0}}{t}\p{x,t}
      - \grad[x] \cdot \paren{\kappa \, \grad[x] w_{t}\sqparen{\delta
          \pi_0}}\p{x, t} + \\
      & + u(x; \pi_0) \cdot \grad[x]{w_{t}\sqparen{\delta
          \pi_0}}\p{x,t}
      = 0
    \end{split}
  \end{equation}
  with homogeneous zero boundary conditions and initial condition,
  \begin{equation}
    w_t \sqparen{\delta \pi_0} \p{x, t_0} = \delta \pi_0, \text{ for }
    x \in \Omega.
  \end{equation}
  The Gateaux Derivatives of $u$ and $p$ are zero.
\end{lemma}
\begin{IEEEproof}
  Since the equation~\eqref{eq:temp} is weakly coupled with the
  fluid's flow equations~\eqref{eq:ns1} and~\eqref{eq:ns2}. The
  variation of initiation condition, $\pi_0$, does not influence $u$
  and $p$. Thus their related derivatives are zeros.

  Then we study $w_{t}\sqparen{\delta \alpha}$,
  Define
  $\tilde{T_e}\p{x,t} = T_e(x,t; \pi_0 + s \delta \pi_0) - T_e(x,t; \pi_0) -
  sw_{t}\p{x,t}$,
  it is sufficient to show that
  \begin{equation}
    \label{eq:lim_wt_pi}
    \lim_{s \to 0} \parenB{ \frac{ \norm{\tilde{T_e}}_{L^2(0,T; H^1(\Omega))} }{ |s| } } = 0
  \end{equation}
  $\tilde{T_e}$ satisfies
  \begin{equation}
    \label{eq:tilde_t_i0}
    \begin{split}
      & \pderiv{\tilde{T_e}}{t}\p{x,t}
      - \grad[x] \cdot \paren{ \kappa \grad[x]{\tilde{T_e}} }\p{x,t} \
      + \\
      & - u(x; \alpha) \cdot \grad[x] \tilde{T_e}\p{x,t}
      = 0
    \end{split}
  \end{equation}
  with zero boundary and initial conditions.

  Since $\tilde{T_e}$ is the solution to the parabolic PDE
  equation~\eqref{eq:tilde_t_i0} with zero boundary and initial
  conditions,
  then according to Lemma~\ref{lem:sigma1_bound}
  and~\ref{lem:sigma1_coercive} and Theorem 11.1.1
  in~\cite{quarteroni2008numerical},
  the only solution, $\tilde{T_e}$, is zero.
  Thus the limitation in equation~\eqref{eq:tilde_t_i0} holds,
  and $w_t\sqparen{\delta \pi_0}$ is the target Gateaux Derivative.
\end{IEEEproof}

\begin{IEEEproof}[Proof of theorem~\ref{thm:frechet}]
  First, we focus on the Fr\'echet derivatives of $J$ with respect to
  $\theta$ as equation~\eqref{eq:theta_deriv}.  
  As a result of lemma~\ref{lem:kappa_derivative},
  according to the chain rule we have the Gateaux derivative of cost
  function, $J$, w.r.t. $\kappa$ in direction $\delta \kappa$ as,
  \begin{equation}
    \label{eq:chain_k}
    \begin{split}
      & \dprodb{\mathcal{D}_{\kappa} J}{\delta \kappa}_{\Omega}
      = \dprod{\pderiv{J}{T_e}}{w_t[\delta \kappa]}_{\Omega \times
        \sqparen{t_0, t_0'}} + \\
      & + \dprod{\pderiv{J}{u}}{w_u[\delta \kappa]}_{\Omega} + \\
      & + \dprod{\pderiv{J}{p}}{w_p[\delta \kappa]}_{\Omega}
      = \dprod{\pderiv{J}{T_e}}{w_t[\delta \kappa]}_{\Omega \times \sqparen{t_0,
          t_0'}}
      + \\
      & + \langle \lambda_1,
                  \pderiv{w_t\sqparen{\delta \kappa}}{t}
                  - \grad[x] \cdot \pb{\delta \kappa \, \grad[x]{T_e}}
      + \\
      & - \grad[x] \cdot \pb{\kappa \, \grad[x]{w_t\sqparen{\delta \kappa}}}
        + u(x) \cdot \grad[x]{w_t\sqparen{\kappa}}
      \rangle_{\Omega \times
        \sqparen{t_0, t_0'}}
      + \\
      & + \dprod{\lambda_4}{w_t\sqparen{\kappa}}_{\partial \Omega \times
        \sqparen{t_0, t_0'}}
      + \dprod{\lambda_6}{w_t\sqparen{\kappa}(x,0)}_{\Omega}
      = \\
      & = \int_{t_0}^{t'_0} \dprodb{\grad[x]{\lambda_1} \cdot \grad[x]{T_e}}{\delta
        \kappa}_{\Omega}\, \mathrm{d}t,
    \end{split}
  \end{equation}
  where $\lambda_{1,4,6}$ are adjoint variables with
  equations~\eqref{eq:ad_pde1} to~\eqref{eq:ad_pde3}.

  Then similar to the equation~\eqref{eq:chain_k}, based on
  lemma~\ref{lem:alpha_derivative} and~\ref{lem:pi0_derivative},
  with the help with adjoint variables,
  we can show the Gateaux derivative of cost function, $J$, w.r.t. $\alpha$ in
  direction $\delta \alpha$.
  %% can be derived as shown in
  %% equation~\eqref{eq:alpha_kappa_deriv},
  %% also the Gateaux derivative of cost function, $J_e$, w.r.t. $\pi_0$ in
  %% direction $\delta \pi_0$ can be derived as shown in
  %% equation~\eqref{eq:theta_i0_deriv}.
  Then by the chain rule, the Gateaux derivatives of $J$
  w.r.t. $\theta$ in direction $\delta \theta$ can be shown as
  equation~\eqref{eq:theta_deriv}.

  Then we extend the derivative in equation~\eqref{eq:theta_deriv}
  above to Fr\'echet derivatives. 
  It is sufficient to show they are linear and bounded.
  Since ajoint variables are not related to variations, the derivative
  in equation~\eqref{eq:theta_deriv} is linear w.r.t. variations.
  In order to show the derivative is bounded, it is sufficient
  to show all the adjoint variables are bounded.
  Since the adjoint variables satisfies the linear PDE system of
  equations~\eqref{eq:ad_pde1} to~\eqref{eq:ad_pde3} and related
  boundary initial conditions in section~\ref{sec:adj_eq},
  according to the energy study for linear PDEs on the Theory
  7.4.1~\cite{quarteroni2008numerical},
  the adjoint variables are bounded.

  Thus the derivative in equation~\eqref{eq:theta_deriv} is Fr\'echet
  derivative.

  Similarly we could show derivatives in
  equation~\eqref{eq:i0_deriv},~\eqref{eq:gte_deriv}
  and~\eqref{eq:gu_deriv} are Fr\'echet derivatives as well.
\end{IEEEproof}

%% \begin{theorem}
%%   \label{thm:jc_frechet}
%%   Given variables,
%%   $g_{T_e} \in L^2 \p{[t_0, t_0'] \times \Omega}$
%%   and $g_u \in L^2 \p{\Omega} \times L^2 \p{\Omega}$,
%%   the directional derivatives in
%%   equation~\eqref{eq:gte_gu_deriv}
%%   are Fr\'echet derivatives of cost function $J_c$ to corresponding variables.
%% \end{theorem}
%% The process to prove the theorem~\ref{thm:jc_frechet} is similar to
%% the proof of the theorem~\ref{thm:je_frechet}, thus we skip it in this
%% appendix.


==> sections/lagrange_existence.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%%%%%%%%%%%%%%%%%%%%%%%
\section{Existence of Lagrange Multipliers}
\label{appendix:existence_lagrange}

\todo{this section needs a lot of work, way more than I'm willing to invest. Is there a good reason to keep it in the appendix? what is shown here that is not included in \cite[Theorem 1.17]{ito2008lagrange}?}

In this section we show the existence of Lagrange multipliers to our optimization problems in eqs.~\eqref{eq:cost_estimate} and~\eqref{eq:cost_control}.

First, we focus on the estimation problem in eq.~\eqref{eq:cost_estimate}.
Let $C_e = \set{(\pi_0, \theta) \in H^1\p{\Omega} \times \sp{0,1}^{n_d}}$.
Also, let us define the space of weak solutions to eqs.~\eqref{eq:temp} to~\eqref{eq:bnd_u1} as:
\begin{equation}
  X = L^2\pb{[t_0, t_0']; H^1(\Omega)} \times \pb{H^1(\Omega) \times H^1(\Omega)} \times L^2(\Omega),
\end{equation}
and consider the space of dual variables:
\begin{multline}
  Z = \setB{L^2\pb{[t_0, t_0']; H^1(\Omega)} \times \pb{H^{-1}(\Omega) \times H^{-1}(\Omega)} \times\\
    \times L^2(\Omega) \times H^1(\Omega) \times L^2(\bdry{\Omega}) \times L^2(\bdry{\Gamma})}.
\end{multline}

Let $\mathcal{S}_e\colon X \times C_e \to Z$ such that:%, for each tuple $\p{T_e, u, p, \pi_0, \theta} \in X \times C_e$, the mapping:
\begin{equation}
  \mathcal{S}_e\p{T_e, u, p, \pi_0, \theta} = \p{v_1, v_2, v_3, v_4, v_5, v_6} \in Z,
\end{equation}
is defined by the following identities for each $\xi \in H_0^1(\Omega)$, $\phi \in H_0^1(\Omega) \times H_0^1(\Omega)$, and $\psi \in L^2(\Omega)$: \todo{this definition is sketchy at best. Is there a reference we can throw in here to avoid drama?}
\begin{multline}
  \label{eq:mp_te}
    \dprodB{\pderiv{T_e(x, t)}{t}}{\xi(x)}_{\Omega}
    - \dprodb{\diver[x]{\pb{\kappa(x,\theta)\, \grad[x]{T_e}(x,t)}}}{\xi(x)}_{\Omega} + \\
    + \dprodb{u(x) \cdot \grad[x]{T_e}(x,t)}{\xi(x)}_{\Omega}
    - \dprodb{g_{T_e}(x,t)}{\xi(x)}_{\Omega} = \\
    = \dprodb{v_1(x,t)}{\xi(x)}_{\Omega}, \quad \forall (x,t) \in \Omega \times [t_0,t_0'].
\end{multline}
\begin{multline}
  \label{eq:mp_u}
  \dprodb{\alpha(x,\theta)\, u(x)}{\phi(x)}_{\Omega}
  + \frac{1}{\reno}\, \dprodb{\grad[x]{u}(x)}{\grad[x]{\phi}(x)}_{\Omega} + \\
  + \dprod{u(x) \cdot \grad[x]{u}(x)}{\phi(x)}_{\Omega}
  - \dprod{p(x)}{\diver[x]{\phi}(x)}_{\Omega} +\\
  - \dprod{g_u(x)}{\phi(x)}_{\Omega}
  = \dprod{v_2(x)}{\phi(x)}_{\Omega}, \quad \forall x \in \Omega.
\end{multline}
\begin{equation}
  \label{eq:mp_p}
  \dprod{\diver[x]{u}(x)}{\psi(x)}_{\Omega}
  = \dprod{v_3(x)}{\psi(x)}_{\Omega},\quad \forall x \in \Omega.
\end{equation}
\begin{equation}
  \label{eq:init_v4}
  T_e(x,t_0) - \pi_0(x)
  = v_4(x), \quad \forall x \in \Omega.
\end{equation}
\begin{equation}
  \label{eq:bnd_v5}
  T_e(x) - T_A
  = v_5(x), \quad \forall x \in \bdry{\Omega},
\end{equation}
\begin{equation}
  \label{eq:bnd_v1}
  u(x) = v_6(x), \quad \forall x \in \bdry{\Omega}.
\end{equation}

%% \begin{equation}
%%   \begin{split}
%%     & \frac{\partial T_e \p{x, t}}{\partial t}
%%     - \grad[x]{} \cdot \parenB{ \kappa\p{x, \theta} \grad T_e
%%       \p{x,t} }
%%     + u \p{x} \cdot \grad[x]{T_e} \p{x,t} + \\
%%     & - g_{T_e}\p{x,t}
%%     = v_1,
%%     \ \ \forall \xi \p{x} \in H^{1}\p{\Omega},
%%   \end{split}
%%   \label{eq:mp_te}
%% \end{equation}
%% \begin{equation}
%%   \begin{split}
%%   & \alpha\p{x, \theta} u \p{x}, \phi \p{x} \rangle_{\Omega}
%%     - \frac{1}{Re} \lapl[x]{u}\p{x}
%%     + u \p{x} \cdot \grad[x]{u\p{x}} + \\
%%   & - \grad[x]{p} \p{x}
%%     - g_u\p{x} = v_2,
%%     \, \, \forall \phi \p{x} \in H^{1}\p{\Omega} \times H^{1}\p{\Omega},
%%   \end{split}
%%   \label{eq:mp_u}
%% \end{equation}
%% \begin{equation}
%%   \grad[x]{\cdot u\p{x}}
%%   = v_3,
%%   \ \ \forall \psi\p{x} \in L^{2}\p{\Omega}
%%   \label{eq:mp_p}
%% \end{equation}
%% \begin{equation}
%%   \label{eq:init_v4}
%%   T_e(x, t_0) - \pi_0(x) = v_4, \quad \text{for}\ x \in \Omega.
%% \end{equation}
%% \begin{equation}
%%   \label{eq:bnd_v5}
%%   T_e(x) - T_A = v_5, \quad \text{for}\ x \in \bdry{\Omega}, \text{
%%     and }
%% \end{equation}
%% \begin{equation}
%%   \label{eq:bnd_v1}
%%   u(x) = v_6, \quad \text{for}\ x \in \Gamma_w.
%% \end{equation}

Note that using the definition above, the weak solutions to eqs.~\eqref{eq:temp} to~\eqref{eq:bnd_u1} satisfy the equality $\mathcal{S}_e(T_e, u, p, \pi_0, \theta) = 0$.

Suppose $\p{T_e^{\star}, u^{\star}, p^{\star}, \pi_0^{\star}, \theta^{\star}}$ is the optimal argument to the problem in~\eqref{eq:cost_estimate}.
Let us define the first derivative of $S_e$ with respect to $X$ at the optimal point as $\mathcal{S}_{e,x^{\star}}'\colon X \rightarrow Z$.
Given $\p{w_t, w_u, w_p} \in X$, the mapping $\mathcal{S}_{e,x^{\star}}'\p{w_{t}, w_{u}, w_p} = \p{v_1, v_2, v_3, v_4, v_5, v_6}$ is defined for each $\xi \in H_0^1(\Omega)$, $\phi \in H_0^1(\Omega) \times H_0^1(\Omega)$, and $\psi \in L^2(\Omega)$ by: \todo{same as above, do we have a reference?}
\begin{multline}
  \label{eq:sD_v1}
  \hspace{-1em}
  \dprod{\pderiv{w_t(x,t)}{t}}{\xi(x)}_{\Omega}
  - \dprodb{\diver[x]{\pb{\kappa^{\star}(x,\theta)\, \grad[x]{w_t}(x,t)}}}{\xi(x)}_{\Omega} + \\
  + \dprodb{u^{\star}(x) \cdot \grad[x]{w_t}(x,t)}{\xi(x)}_{\Omega} + \\
  + \dprodb{w_u(x) \cdot \grad[x]{T_e^{\star}}(x,t)}{\xi(x)}_{\Omega}
  = \dprodb{v_1(x)}{\xi(x)}_{\Omega}, \ \forall x \in \Omega.
\end{multline}
\begin{multline}
  \label{eq:sD_v2}
  \dprodb{\alpha(x,\theta)\, w_u(x)}{\phi(x)}_{\Omega}
  + \frac{1}{\reno}\, \dprodb{\grad[x]{w_u}(x)}{\grad[x]{\phi}(x)}_{\Omega} + \\
  + \dprodb{w_u(x) \cdot \grad[x]{u^{\star}}(x)}{\phi(x)}_{\Omega}
  + \dprodb{u^{\star}(x) \cdot \grad[x]{w_u}(x)}{\phi(x)}_{\Omega} +\\
  - \dprodb{w_p(x)}{\diver[x]{\phi}(x)}_{\Omega}
  = \dprodb{v_2(x)}{\phi(x)}_{\Omega}, \quad \forall x \in \Omega.
\end{multline}
\begin{equation}
  \label{eq:sD_v3}
  \dprodb{\diver[x]{w_u}(x)}{\psi(x)}_{\Omega}
  = \dprodb{v_3(x)}{\psi(x)}_{\Omega}, \quad \forall x \in \Omega.
\end{equation}
\begin{equation}
  \label{eq:sD_v4}
  w_t(x,t_0) = v_4(x), \quad \forall x \in \Omega.
\end{equation}
\begin{equation}
  \label{eq:sD_v5}
  w_t(x) = v_5(x), \quad \forall x \in \bdry{\Omega},
\end{equation}
\begin{equation}
  \label{eq:sD_v6}
  w_u(x) = v_6(x), \quad \forall x \in \bdry{\Omega}.
\end{equation}

\begin{lemma}
  \label{lem:sD_closed}
  $\mathcal{S}_{e,x^{\star}}'$ is a closed operator.
\end{lemma}
\begin{IEEEproof}
  Since $\mathcal{S}_{e,x^{\star}}'$ is a linear operator with respect to $\p{w_t, w_u, w_p}$ \todo{citation missing}, it is sufficient to show that, for an arbitrary sequence in $X$ converging to $0$, say $\set{(w_{t,i}, w_{u,i},  w_{p,i})}_{i=1}^{\infty}$, then $\mathcal{S}_{e,x^{\star}}'(w_{t,i}, w_{u,i}, w_{p,i}) \rightarrow 0$.
  But, as shown in Appendix~\ref{appendix:existence} and the Lax-Milgram Theorem~\cite[Chapter~1.2]{girault2012finite}, the only solution to $\mathcal{S}_{e,x^{\star}}' = 0$ is $\p{w_t, w_u, w_p} = 0$, thus operator $\mathcal{S}_{e,x^{\star}}^{'}$ is closed. \todo{this statement is completely insufficient as a proof. Do we have a reference so we don't have to write this proof?}
\end{IEEEproof}

\begin{lemma}
  \label{lem:sD*_surjective}
  Let $\widehat{\mathcal{S}}_{e,x^{\star}}'\colon Z^{\star} \to X^{\star}$ be the adjoint operator of $\mathcal{S}_{e,x^{\star}}'$.
  Then $\widehat{\mathcal{S}}_{e,x^{\star}}'$ is surjective.
\end{lemma}
\begin{IEEEproof}
  Since $\mathcal{S}_{e,x^{\star}}'$ is closed and its domain is the space $X$, then it is sufficient to show that the kernel of $\mathcal{S}_{e,x^{\star}}'$ is the null set \todo{citation missing}.
  The result follows trivially since this is exactly what was shown in the proof of Lemma~\ref{lem:sD_closed}.
\end{IEEEproof}

\begin{lemma}
  \label{thm:estimate_lg}
    If $\p{T_e^{\star}, u^{\star}, p^{\star}, \pi_0^{\star}, \theta^{\star}}$ is the optimal argument to the problem in eq.~\eqref{eq:cost_estimate}, then there exist Lagrange multipliers, denoted $\set{\lambda_i}_{i=1}^6$, satisfying the following weak PDEs for each $(w, v, q) \in L^2\pb{[t_0, t_0']; H^1(\Omega)} \times \pb{H^1(\Omega) \times H^1(\Omega)} \times L^2(\Omega)$:
  \begin{multline}
    - \pderiv{J}{T_e} + \pderiv{\lambda_1}{t}(x,t) + \diver[x]{\pb{\kappa(x)\, \grad[x]{\lambda_1}(x,t)}} +\\
      + u(x) \cdot \grad[x]{\lambda_1}(x,t) = 0,
  \end{multline}
  \begin{equation}
    \lambda_6(x) = \lambda_1\p{x,0},
  \end{equation}
  \begin{multline}
    \int_{t_0}^{t_0'} \lambda_1(x,t)\, \grad[x]{T_e}(x,t)\, \diff{t} + \alpha(x)\, \lambda_2(x) - \frac{1}{\reno}\, \lapl[x]{\lambda_2}(x) + \\
    - u(x) \cdot \grad[x]{\lambda_2}(x) + \lambda_2(x) \cdot \grad[x]{u}(x) - \grad[x]{\lambda_3}(x) = 0,
  \end{multline}
  \begin{equation}
    \diver[x]{\lambda_2}(x) = 0,
  \end{equation}
  with boundary conditions $\lambda_1(x,t) = 0$ and $\lambda_2(x) = 0$ for each $x \in \bdry{\Omega}$ and $t \in [t_0, t_0']$, together with final condition $\lambda_1\p{x,T} = 0$ for each $x \in \Omega$.
  % The adjoint functions $\lambda_4$ and $\lambda_5$ are irrelevant to our Fr\'echet derivative calculation, therefore we omit them from this presentation.

  %%%%%%%%%%% I'm here editing. Continuing is rather pointless since none of these results comes attached to a real proof.

  If $\p{T_e^{\star}, u^{\star}, p^{\star}, g_{T_e}^{\star}, g_u^{\star}}$ is the optimal point to the problem in eq.~\eqref{eq:cost_control}, its Lagrange multipliers, $\lambda_{1,2,3,6}$, also satisfy the above ajoint PDE system.
\end{lemma}
\begin{IEEEproof}
  According to subsection~\ref{appendix:frechet_proof}, $\p{T_e, u, p}$ are
  Gateaux differentiable w.r.t. $\p{\theta, \alpha, \kappa, \pi_0}$.
  Furthermore, according to Lemma~\ref{lem:sD_closed} and~\ref{lem:sD*_surjective},
  $\mathcal{S}_{e, x^{\star}}^{'}$ is continuous and
  $\mathcal{S}_{e, x^{\star}}^{', \star}$ is surjective,
  then the Lagrange multipliers exist.
  According to~\cite{he2016gradient},
  the Lagrange multipliers, $\{\lambda_i\}_{i = 1,2,3, 6}$ satisfy
  equations~\eqref{eq:ad_pde1},~\eqref{eq:ad_pde2} and~\eqref{eq:ad_pde3}
  hold~\cite[Theorem 1.17]{ito2008lagrange}.

  Similarly, we can prove the existence of Lagrange multipliers to the
  problem~\ref{eq:cost_control}.
\end{IEEEproof}
%% For the control problem in equation~\eqref{eq:cost_control},
%% with similar strategy we have,
%% \begin{theorem}
%%   \label{thm:control_lg}
%%   If $\p{T_e^{\star}, u^{\star}, p^{\star}, g_{T_e}^{\star}, g_u^{\star}}$ is the optimal
%%   point to the problem~\eqref{eq:cost_control},
%%   then there exist Lagrange multipliers, $\{\lambda_i\}_{i=1}^6$,
%%   which are corresponding to PDE-constraints,
%%   such that $\forall \p{w, v, q}
%%   \in L^2{\sqparen{t_0, t_0'}; H^1\p{\Omega}} \times \pb{H^1\p{\Omega}
%%     \times H^1\p{\Omega}} \times L^2\p{\Omega}$,
%%   the Lagrange function's variation w.r.t. $\p{w, v, q}$ is zero, and
%%   $\lambda_{1,2,3,6}$ satisfy the PDE equations and boundary and final
%%   condition in theorem~\ref{thm:estimate_lg1}.
%% \end{theorem}


==> sections/opt_convergence.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%%%%%%%%%%%%%%%%%%%%%%%
\section{Convergence of the Algorithm}
\label{appendix:convergence}
%% In this section we are going to show the convergence of the
%% algorithms~\ref{alg:grd_est} in section~\ref{subsec:grad_method}.
%% \begin{theorem}
%%   Suppose the cost functions in problem~\eqref{eq:cost_estimate} and~\eqref{eq:cost_control}
%%   are bounded from below,
%%   and $\beta_e, \beta_c \in \p{0, 1}$ in algorithm~\ref{alg:grd_est}
%%   and~\ref{alg:grd_control} satisfy respectively,
%%   when $V_e \p{\theta, \pi_0}, V_c \p{g_{T_e}, g_u} < 0$,
%%   $a \in \p{0, 1}$
%%   \begin{equation}
%%     J_e\p{\theta + \beta_e \delta \theta, \pi_0 + \beta_e \delta \pi_0}
%%     - J_e \p{\theta, \pi_0}
%%     \leq a \, \beta_e V_e \p{\theta, \pi_0},
%%     \label{eq:uni_descent_1}
%%   \end{equation}
%%   \begin{align}
%%     \begin{split}
%%     & J_c \p{g_{T_e} + \beta_c \delta g_{T_e}, g_u + \beta_c \delta g_u}
%%     - J_c \p{g_{T_e}, g_u} \leq \\
%%     & \leq a \, \beta_c V_c \p{g_{T_e}, g_u}.
%%     \end{split}
%%     \label{eq:uni_descent_2}
%%   \end{align}

%%   where $\p{\delta \theta, \delta \pi_0}$ are
%%   derived from problem~\eqref{eq:qp_grad_estimate},
%%   $\p{\delta g_{T_e}, \delta g_u}$ are derived from problem~\eqref{eq:qp_grad_control}.
%%   Then for arbitrary sequence generated by the
%%   algorithm~\ref{alg:grd_est} or~\ref{alg:grd_control},
%%   its accumulate point satisfies $V_e \p{\pi_0, \theta} = 0$ or
%%   $V_c \p{g_{T_e}, g_u} = 0$.
%%   \label{thm:algorithm_converge_estimation}
%% \end{theorem}
\begin{IEEEproof}{Proof of theorem~\ref{thm:algorithm_converge}}
  It is trivial to show that $V_e \p{\pi_0, \theta}$ and $V_c
  \p{g_{T_e}, g_u}$ are optimality functions.
  And under the assumption in equations~\eqref{eq:armijo_estimate}
  and~\eqref{eq:armijo_control}, 
  the updating step satisfies the uniform sufficient descent property.
  Thus using the same contradiction strategy in~\cite[Theorem
    5.12]{Vasudevan2013a}, 
  the accumulate point of every sequence generated by
  algorithm in Fig.~\ref{fig:algo} satisfy
  %% algorithm~\ref{alg:grd_est} and~\ref{alg:grd_control} satisfies
  $V_e \p{\pi_0, \theta}= 0$ and $V_c \p{g_{T_e}, g_u} = 0$ respectively.
\end{IEEEproof}

